Verifying the Smallest Interesting Colour Code with Quantomatic

In this paper we present a Quantomatic case study, verifying the basic properties of the Smallest Interesting Colour Code error detecting code.

==> eptcsdata.tex <==
\providecommand{\firstpage}{147}
\providecommand{\publicationstatus}{Bob Coecke and Aleks Kissinger (Eds.):\\ 14th International Conference on Quantum Physics and Logic (QPL)\\
EPTCS 266, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.266.10}{10.4204/EPTCS.266.10}}
\pdfoutput=1

